Efficient algorithms for optimal homology problems and their applications

The multiscale simplicial flat norm (MSFN) of a d-cycle is a family of optimal homology problems indexed by a scale parameter {\lambda} >= 0. Each instance (mSFN) optimizes the total weight of a homologous d-cycle and a bounded (d + 1)-chain, with one of the components being scaled by {\lambda}.We propose a min-cost flow formulation for solving instances of mSFN at a given scale {\lambda} in polynomial time in the case of (d + 1)-dimensional simplicial complexes embedded in {R^(d + 1)} and homology over Z. Furthermore, we establish the weak and strong dualities for mSFN, as well as the complementary slackness conditions. Additionally, we prove optimality conditions for directed flow formulations with cohomology over Z+. Next, we propose an approach based on the multiscale flat norm, a notion of distance between objects defined in the field of geometric measure theory, to compute the distance between a pair of planar geometric networks. Using a triangulation of the domain containing the input networks, the flat norm distance between two networks at a given scale can be computed by solving a linear program. In addition, this computation automatically identifies the 2D regions (patches) that capture where the two networks are different. We demonstrate through 2D examples that the flat norm distance can capture the variations of inputs more accurately than the commonly used Hausdorff distance. As a notion of stability, we also derive upper bounds on the flat norm distance between a simple 1D curve and its perturbed version as a function of the radius of perturbation for a restricted class of perturbations. We demonstrate our approach on a set of actual power networks from a county in the USA. Our approach can be extended to validate synthetic networks created for multiple infrastructures such as transportation, communication, water, and gas networks.

==> abstract/fn-bound-abstract.tex <==
\begin{abstract}
  We study the problem of comparing a pair of geometric networks that may not be similarly defined, i.e., when they do not have one-to-one correspondences between their nodes and edges.
  Our motivating application is to compare power distribution networks of a region.
  Due to the lack of openly available power network datasets, researchers synthesize realistic networks resembling their actual counterparts.
  But the synthetic digital twins may vary significantly from one another and from actual networks due to varying underlying assumptions and approaches.
  Hence the user wants to evaluate the quality of networks in terms of their structural similarity to actual power networks.
  But the lack of correspondence between the networks renders most standard approaches, e.g., subgraph isomorphism and edit distance, unsuitable. % for this purpose.

  We propose an approach based on the \emph{multiscale flat norm}, a notion of distance between objects defined in the field of geometric measure theory, to compute the distance between a pair of planar geometric networks.
  Using a triangulation of the domain containing the input networks, the flat norm distance between two networks at a given scale can be computed by solving a linear program.
  In addition, this computation automatically identifies the 2D regions (patches) that capture where the two networks are different.
  We demonstrate through 2D examples that the flat norm distance can capture the variations of inputs more accurately than the commonly used Hausdorff distance.
  As a notion of \emph{stability}, we also derive upper bounds on the flat norm distance between a simple 1D curve and its perturbed version as a function of the radius of perturbation for a restricted class of perturbations.
  We demonstrate our approach on a set of actual power networks from a county in the USA.
  Our approach can be extended to validate synthetic networks created for multiple infrastructures such as transportation, communication, water, and gas networks.
\end{abstract}


==> appendices/app.tex <==
\appendix

%%%%%%%%%% DON'T DELETE THIS, REVERTS NUMBERING BACK %%%%%%%%%%%%%
\makeatletter
\renewcommand{\@makechapterhead}[1]{\vspace *{-10\p@ }{\parindent \z@ 
\raggedright \normalfont \ifnum \c@secnumdepth >\m@ne \Huge \bfseries 
\@chapapp \space \thechapter \vskip 10\p@ \fi #1\par \nobreak \vskip 30\p@ }}
\makeatother
%%%%%%%%%% DON'T DELETE THIS, REVERTS NUMBERING BACK %%%%%%%%%%%%%


\import{./}{appendix-fn-flow-examples}

%\chapter{MSFN: LP vs MinCostFlow}
%\vspace*{-0.3in}
%\begin{figure}[hb!]
%\begin{center}
%\makebox[\textwidth][c]{\includegraphics[width=1.0\textwidth]{figs/costperMb2015_4.jpg}}
%\end{center}
%\caption[Cost per raw megabase of DNA sequence from 2001 to 2015]{Cost per raw megabase of DNA sequence from 2001 to 2015. Straight line - Moore's Law, blue curve - cost in US dollars, Y-axis scale is logarithmic. Graph reproduced from \citep{wetterstrand2016}}
%\end{figure}

%\chapter{MSFN: Structural Validation Of Synthetic Power Distribution Networks}
%\begin{figure}[hb!]
%\begin{center}
%\includegraphics[scale=0.5]{figs/costperMb2015_4.jpg}
%\end{center}
%\caption[Cost per raw megabase of DNA sequence from 2001 to 2015]{Cost per raw megabase of DNA sequence from 2001 to 2015. Straight line - Moore's Law, blue curve - cost in US dollars, Y-axis scale is logarithmic. Graph reproduced from \citep{wetterstrand2016}}
%\end{figure}


\chapter{Persistent Cycles in Directed Bipartite Graph}

%\import{./}{appendix-react-plots.tex}

%\section{Examples: Super-Fast mechanism}
%\section{Analysis: Distance between persistence diagrams}
%\section{Analysis: Distribution of Cycle Representatives}
%
%\begin{figure}[hb!]
%\begin{center}
%\includegraphics[scale=0.5]{figs/costperMb2015_4.jpg}
%\end{center}
%\caption[Cost per raw megabase of DNA sequence from 2001 to 2015]{Cost per raw megabase of DNA sequence from 2001 to 2015. Straight line - Moore's Law, blue curve - cost in US dollars, Y-axis scale is logarithmic. Graph reproduced from \citep{wetterstrand2016}}
%\end{figure}



%\chapter{Other appendix}
%\begin{figure}[hb!]
%\begin{center}
%\includegraphics[scale=0.5]{figs/costperMb2015_4.jpg}
%\end{center}
%\caption[Cost per raw megabase of DNA sequence from 2001 to 2015]{Cost per raw megabase of DNA sequence from 2001 to 2015. Straight line - Moore's Law, blue curve - cost in US dollars, Y-axis scale is logarithmic. Graph reproduced from \citep{wetterstrand2016}}
%\end{figure}



==> chapters/chapter-01/fn-bound-intro.tex <==
% \section{Introduction}\label{sec:intro:fn-bound}

% What is digital twin of a power grid and why do we need it?
The power grid is the most vital infrastructure that provides crucial support for the delivery of basic services to most segments of society.
Once considered a passive entity in power grid planning and operation, the power distribution system poses significant challenges in the present day.
The increased adoption of rooftop solar photovoltaics (PVs) and electric vehicles (EVs) augmented with residential charging units has altered the energy consumption profile of an average consumer.
Access to extensive datasets pertaining to power distribution networks and residential consumer demand is vital for public policy researchers and power system engineers alike.
However, the proprietary nature of power distribution system data hinders their public availability.
This has led researchers to develop frameworks that synthesize realistic datasets pertaining to the power distribution system~\cite{highres_net,overbye_2020,nrel_net,rounak2020,anna_naps,schweitzer}.
These frameworks create digital replicates similar to the actual power distribution networks in terms of their structure and function.
Hence the created networks can be used as \emph{digital duplicates} in simulation studies of policies and methods before implementation in real systems.

%what is structural validation; example of where structural comparison becomes important
The algorithms associated with these frameworks vary widely---ranging from first principles based approaches~\cite{rounak2020,anna_naps} to learning statistical distributions of network attributes~\cite{schweitzer} to using deep learning models such as generative adversarial neural networks~\cite{feeder_gan}.
Validating the synthetic power distribution networks with respect to their physical counterpart is vital for assessing the suitability of their use as effective digital duplicates.
Since the underlying assumptions and algorithms of each framework are distinct from each other, some of them may excel compared to others in reproducing digital replicates with better precision for selective regions.
To this end, we require well-defined metrics to rank the frameworks and judge their strengths and weaknesses in generating digital duplicates of power distribution networks for a particular geographic region.

The literature pertaining to frameworks for synthetic distribution network creation include certain validation results that compare the generated networks to the actual counterpart~\cite{highres_net,validate2020,schweitzer}. But the validation results are mostly limited to comparing the statistical network attributes such as degree and hop distributions and power engineering operational attributes such as node voltages and edge power flows. Since power distribution networks represent real physical systems, the created digital replicates have associated geographic embedding. Therefore, a structural comparison of synthetic network graphs to their actual counterpart becomes pertinent for power distribution networks with geographic embedding.
Consider an example where a digital twin is used to analyze impact of a weather event~\cite{samiul2021}.
Severe weather events such as hurricanes, earthquakes and wild fires occur in specific geographic trajectories, affecting only portions of societal infrastructures.
In order to correctly identify them during simulations, the digital twin should structurally resemble the actual infrastructure.

\medskip
\noindent\textbf{Problem Statement:} 
In recent years, the problem of evaluating the quality of reconstructed networks has been studied for street maps.
Certain metrics were defined to compare outputs of frameworks that use GPS trajectory data to reconstruct street map graphs~\cite{roads_2015,roads2014}.
The abstract problem can be stated as follows: \emph{compute the similarity between a given pair of embedded planar graphs}.
This is similar to the well known subgraph isomorphism problem~\cite{eppstein_1995} wherein we look for isomorphic subgraphs in a pair of given graphs.
A major precursor to this problem is that we require a one-to-one mapping between nodes and edges of the two graphs.
While such mappings are well-defined for street networks, the same cannot be inferred for power distribution networks.
Since power network datasets are proprietary, the node and edge labels are redacted from the network before it is shared.
The actual network is obtained as a set of ``drawings'' with associated geographic embeddings. Each drawing can be considered as a collection of line segments termed a \emph{geometry}. Hence the problem of comparing a set of power distribution networks with geographic embedding can be stated as the following: 
\emph{compute the similarity between a given pair of geometries lying on a geographic plane}.

\medskip
\noindent\textbf{Our Contributions:} 
We propose a new distance measure to compare a pair of geometries using the \emph{flat norm}, a notion of distance between generalized objects studied in geometric measure theory~\cite{Federer1969,Morgan2016}.
This distance combines the difference in length of the geometries with the area of the patches contained between them. The area of patches in between the pair of geometries accounts for the lateral displacement between them.
%Hence, this combination ensures that all possible deviations are accounted for a pair of geometries embedded on the same plane.
We employ a \emph{multiscale} version of the flat norm~\cite{MoVi2007} that uses a scale parameter $\lambda \geq 0$ to combine the length and area components
(for the sake of brevity, we refer to the multiscale flat norm simply as the flat norm).
Intuitively, a smaller value of $\lambda$ captures larger patches of area between the geometries while a large value of $\lambda$ captures more of the (differences in) lengths of the geometries.
Computing the flat norm over a range of values of $\lambda$ allows us to compare the geometries at multiple scales.
For computation, we use a discretized version of the flat norm defined on simplicial complexes~\cite{ibrahim2011simplicial}, which are triangulations in our case.
% The scale parameter $\lambda$ allows us to compute the simplicial flat norm at various scales of sets defined as oriented subcomplexes in arbitrary dimensions.
It may not be possible to derive standard stability results for this distance measure that imply only small changes in the flat norm metric when the inputs change by a small amount---there is no alternative metric to measure the \emph{small change in the input}.
We demonstrate through 2D examples (in Fig.~\ref{fig:currents:example-currents-and-neighborhoods}), for instance, that the commonly used Hausdorff metric cannot be used for this purpose.
Instead, we have derived upper bounds on the flat norm distance between a piecewise linear 1-current and its perturbed version as a function of the radius of perturbation under certain assumptions provided the perturbations are performed carefully (see Section \ref{subsec:FN-BOUND}).

A lack of one-to-one correspondence between edges and nodes in the pair of networks prevents us from performing one-to-one comparison of edges.
Instead we can sample random regions in the area of interest and compare the pair of geometries within each region.
For performing such local comparisons, we define a \emph{normalized flat norm} where we normalize the flat norm distance between the parts of the two geometries by the sum of the lengths of the two parts in the region. 
Such comparison enables us to characterize the quality of the digital duplicate for the sampled region.
Further, such comparisons over a sequence of sampled regions allows us to characterize the suitability of using the entire synthetic network as a duplicate of the actual network. 

Our \textbf{main contributions} are the following:
(i) we propose a distance measure for comparing a pair of geometries embedded in the same plane using the flat norm that accounts for deviation in length and lateral displacement between the geometries; and
(ii) we perform a region-based characterization of synthetic networks by sampling random regions and comparing the pair of geometries contained within the sampled region.
The proposed distance allows us to perform global as well as local comparisons between a pair of network geometries.



==> chapters/chapter-01/intro-cgyrf.tex <==
%>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>
%\section{Introduction (CGYRF)}
%\label{sec:cgyrf:intro}
%>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>


The \emph{flat norm} is a tool from geometric measure theory to measure distances between shapes~\cite{glaunes2005transport, meyur2023structural}.
The \embf{multiscale Simplicial Flat Norm (mSFN)} \cite{ibrahim2011simplicial,  vixie2010multiscale}, 
is a discretization of the flat norm to spaces triangulated by a simplicial complex.
 In general, mSFN is NP-hard even when homology is defined over integers, however in the case of embedded complexes it can be solved in polynomial time, for example as a linear relaxation of an integer program \cite{ibrahim2011simplicial}, which at best has matrix multiplication time {$O(n^{2.38} \log n)$}\cite{van2020deterministic}.
Here we propose a network flow model for solving mSFN as a min-cost flow on the dual graph of a $(d + 1)$-simplicial complex embedded in $\real^{d + 1}$. 
The fastest algorithm for solving min-cost problems at the time of writing
has almost linear complexity $m^{1 + o(1)}$ in terms of the number of edges, \cite{chen2022maximum}.

Let $\mc{K}$ be a $d$-connected orientable $(d + 1)$-dimensional simplicial complex embedded in $\real^{d + 1}$ 
with $\beta_{d} + 1$ boundary components, 
that correspond to the connected components $\real^{d + 1} \setminus \supp(\mc{K})$ that we call \emph{voids}, let $\nu_{0}$ be the  unbounded one.
The non-negative weights assigned to the $d$-simplices $e_{i} \in \mc{K}_{d}$ by the \embf{length-volume} function ${c}\!: \mc{K}_{d} \to \integerplus$, 
and to the $(d + 1)$-simplices $\tau_{j} \in \mc{K}_{d + 1}$ by the \embf{area-volume} ${a}\!: \mc{K}_{d + 1} \to \integerplus$, respectively. 
The homomorphisms $\bd_{d + 1}\!: \mc{C}_{d + 1}(\mc{K}) \to \mc{C}_{d}(\mc{K})$ and $\cobd_{d + 1}: \mc{C}^{d}(\mc{K}) \to \mc{C}^{d + 1}(\mc{K})$ 
are the  \embf{boundary } and the \embf{coboundary operators} respectively.
We assume that its simplices are oriented, we associate the positive orientation with the \emph{clockwise} direction.
Let's say that $\bd_{d + 1} \tau (e) = +1$ and $\bd_{d + 1} \eta (e) = -1$,
then we write  $\cobd_{d + 1} e = \tau - \eta$.
Let $\bm{z} \in \mc{Z}_{d}(\mc{K}; \integer)$ be an input $d$-cycle on $\mc{K}$.
Two $d$-cycles $\bm{z}$ and $\bm{x}$ are said to be \embf{homologous}, denoted as $\bm{z} \sim \bm{x}$,
if for some $(d + 1)$-chain $\bm{\pi}$: $\bd_{d + 1} \bm{\pi} = \bm{z} - \bm{x}$.


\begin{definition}[MSFM]
    Given a scale parameter $\lambda \in \integerplus$,
    the \embf{multiscale simplicial flat norm} of $\bm{z} \in \mc{Z}_{d}(\mc{K}; \integer)$ is defined as a minimization
    \begin{align}
    \label{eq:cgyrf:flat-norm-def}
    %----------------------------------------------------------------------------------------------
        {\mbb{F}}_{\lambda}(\bm{z}) 
         = \min\limits_{\bm{x} \sim \bm{z}} {\mbb{F}}_{\lambda}(\bm{z}; \bm{x}) 
         = \min\limits_{\bm{x} \sim \bm{z}} 
            \big\{ \abs{c({\bm{x}})} + \lambda  \abs{a({\bm{\pi}})} \ \big\vert \  \bd_{d + 1} \bm{\pi} = \bm{z} - \bm{x} \big\}
    %----------------------------------------------------------------------------------------------
    \end{align}
    where $\abs{c({\bm{x}})} = \sum_{\mc{K}_{d}} c_i  \abs{x_i}$ and  $\abs{a({\bm{\pi}})} = \sum_{\mc{K}_{d + 1}} a_j  \abs{\pi_j}$.
    The pair $(\bm{x}_{\star}, \bm{\pi}_{\star})$ that minimizes ${\mbb{F}}_{\lambda}(\bm{z}; \bm{x})$
    is called the \embf{(optimal) flat norm decomposition (FN-decomposition)} of $\bm{z}$.
\end{definition}

Note that due to the embedding assumptions the FN-decomposition of $\bm{z}$ is unique, otherwise $\mc{K}$ should have a non-bounding $(d + 1)$-cycle. 
For brevity, we will consider here $\lambda = 1$, which corresponds to the default \emph{simplicial flat norm} $\mbb{F}(\bm{z})$ of $\bm{z}$.
The following integer linear program computes ${\mbb{F}}(\bm{z})$ in Eq.~\eqref{eq:cgyrf:flat-norm-def} and its dual max-flux program\cite{sullivan1990crystalline}:
\cite{sullivan1990crystalline}
\begin{align}
\label{eq:cgyrf:flat-norm-lp}
%----------------------------------------------------------------------------------------------
    %·······································································
        \begin{array}{rl}\dsp
            \min\limits_{\bm{x}, \bm{\pi}}\ 
            &\dsp  
                    {c}(\bm{x}^{+}) + {c}(\bm{x}^{-}) + {a}(\bm{\pi}^{+}) + {a}(\bm{\pi}^{-})
            \\[2pt]
            %·····················································
            \text{s.t.} &\dsp 
                    \bd_{d + 1} (\bm{\pi}^{+} - \bm{\pi}^{-}) + \bm{x}^{+} - \bm{x}^{-} = \bm{z}         
            \\ 
            %·····················································
            &\dsp 
                    \bm{x}^{\pm}  \geq \bm{0}_{E}, \ \bm{\pi}^{\pm}  \geq \bm{0}_{F}
            %·····················································
        \end{array}
    %·······································································
    &&\overset{dual}{\Longrightarrow}&&
    %·······································································
        \begin{array}{lll}\dsp
            \max\limits_{ \tilde{\bm{f}} }\
            &\dsp 
                    \tilde{\bm{f}}(\bm{z})
            \\[2pt]
            %·····················································
            \text{s.t.} &\dsp  
                    -\bm{a} \leq \cobd_{d + 1} \tilde{\bm{f}} \leq \bm{a}
            \\  
            %·····················································
            &\dsp  
                    -\bm{c} \leq \tilde{\bm{f}} \leq \bm{c}
            %·····················································
        \end{array}
    %·······································································
%----------------------------------------------------------------------------------------------
\end{align}
where the dual variable is a $d$-cochain $\tilde{\bm{f}} \in  \mc{C}^{d}(\mc{K}; \integer)$, 
which we refer to as \embf{$d$-pseudocoflow}.
Recall, that the embedding assumptions guarantee that the boundary matrix $[\bd_{d + 1}]$ is \emph{totally unimodular} \cite{ohcp2011},
and since all weights $\bm{c}$ and $\bm{a}$ are integral, 
we can find an optimal integral solution in \emph{polynomial time} for both programs in Eq.~\eqref{eq:cgyrf:flat-norm-lp}, \cite{veinott1968integral, ibrahim2011simplicial}.

The procedure described in {Algorithm~\ref{algo:cgyrf:flow-network}} extends the dual graph $\mc{K}^{*}$ to the dual flow network $\tilde{\mc{K}}^{*}_{FN}$ by introducing auxiliary source and sink nodes,
such that that any $d$-pseudocoflow has non-positive flux $\tilde{\bm{f}}(\bm{z}) \leq 0$ through $\bm{z}$ and any $\bm{x} \sim \bm{z}$ on $\mc{K}$. 
The rigorous constructions of related chain complexes and proof of equivalence to the original problem are out of the scope of this short abstract and are presented in the accompanying paper.


Let's define $\bm{g} \in \mc{C}^{d + 1} (\mc{K}; \integer)$ 
such that it obeys  the  circulation imbalance conditions: 
$-\bm{a} \leq \bm{g} \leq \bm{a}$ 
and $\cobd_{d + 1} \tilde{\bm{f}} + \bm{g} = 0$ .
Then the fixed max-flux problem from Eq.~\eqref{eq:cgyrf:flat-norm-lp} and its dual:
\begin{align}
\label{eq:cgyrf:flat-norm-fixed}
%----------------------------------------------------------------------------------------------
    %·······································································
        \begin{array}{lll}\dsp
            \max\limits_{ \tilde{\bm{f}}, \bm{g} }\ 
            &\dsp 
                    \tilde{\bm{f}}(\bm{z}) + 0 \cdot \bm{g}
            \\[2pt]
            %·····················································
            \text{s.t.} &\dsp  
                     \tilde{\bm{f}}(\bd_{d + 1} \tau_j) +  \bm{g}(\tau_j) = 0
            \\[2pt]
            %·····················································
            &\dsp  
                    -\bm{c} \leq \tilde{\bm{f}} \leq \bm{c}
            \\[2pt]
            %·····················································
            &\dsp  
                    -\bm{a} \leq \bm{g}  \leq \bm{a}   
            %·····················································
        \end{array}
    %·······································································
    &&\overset{dual}{\Longrightarrow}&&
    %·······································································
        \begin{array}{rl}\dsp
            \min\limits_{\bm{x}, \bm{\pi}, \bm{\psi}}\ 
            &\dsp  
                    0 \cdot \bm{\pi} + 
                    {a}(\bm{\psi}^{+}) + {a}(\bm{\psi}^{-}) + 
                    \abs{{c}({\bm{x}})}
            \\[2pt]
            %·····················································
            \text{s.t.} &\dsp 
                    \bd_{d + 1} \bm{\pi} + \bm{x} = \bm{z}         
            \\[2pt] 
            %·····················································
            &\dsp 
                    \bm{\pi} + \bm{\psi}^{+} - \bm{\psi}^{-} = \bm{0}_{F}         
            \\[2pt] 
            %·····················································
            &\dsp 
                    \bm{\pi} \in \integer^{F}; \ 
                    \bm{\psi}^{\pm} \geq \bm{0}_{F}; \
                    \bm{x}  \in \integer^{E}
            %·····················································
        \end{array}
    %·······································································
%----------------------------------------------------------------------------------------------
\end{align}


\begin{theorem}[Weak and Strong Duality]
    Let $(\bm{x}, \bm{\pi})$ be a feasible solution for the mSFN problem in Eq.~\eqref{eq:cgyrf:flat-norm-lp}
    such that $\bm{x} \sim \bm{z}$ and $\bd_{d + 1} \bm{\pi} = \bm{z} - \bm{x}$,
%    for $\bm{\pi} \in \mc{C}_{d + 1}(\mc{K}; \integer)$,
    and $(\tilde{\bm{f}}, \bm{g})$ be a feasible solution for the Max-Flux problem in Eq.~\eqref{eq:cgyrf:flat-norm-fixed} such that $\tilde{\bm{f}}(\bm{z}) \leq 0$.
    Let $({\bm{x}}_{\star}, \bm{\pi}_{\star})$ and $(\tilde{\bm{f}}_{\star}, {\bm{g}}_{\star})$ be corresponding optimal solutions.
    Then it holds:
    \begin{align}
    %----------------------------------------------------------------------------------------------
    \label{eq:cgyrf:weak-duality}
          &0 \leq \tilde{\bm{f}}(-\bm{z})  
            \leq \tilde{\bm{f}}_{\star}(-\bm{z})  
            \leq \abs{c({\bm{x}_{\star}})} +  \abs{a({\bm{\pi}_{\star}})} 
            \leq \abs{c({\bm{x}})} +  \abs{a({\bm{\pi}})} &
    \\
    %----------------------------------------------------------------------------------------------
%    \end{align}
%    \begin{align}
    %----------------------------------------------------------------------------------------------
    \label{eq:cgyrf:strong-duality}
       & \begin{array}{cclccll}
            %·············································································
            {\bm{x}}_{\star}(e_i) > 0     &\iff& \tilde{\bm{f}}_{\star}(e_i) =  - {c_i} &\qquad&
            \bm{\pi}_{\star}(\tau_j) >0   &\iff& {\bm{g}}_{\star}(\tau_j)    = \me{a_j} \\
            %·············································································
            {\bm{x}}_{\star}(e_i) < 0     &\iff& \tilde{\bm{f}}_{\star}(e_i) = \me{c_i} &\qquad&
            \bm{\pi}_{\star}(\tau_j) < 0  &\iff& {\bm{g}}_{\star}(\tau_j)    =  - {a_j} 
            %·············································································
        \end{array}&
    %----------------------------------------------------------------------------------------------
    \end{align}
\end{theorem}



%===========================================================================================================
% \subsection{Flow network for mSFN}
%===========================================================================================================

%\IncMargin{1em}
% \label{algo:FN-flow-network}
\begin{algorithm}[!p]

     \caption{Flow Network Setup.}
     \label{algo:cgyrf:flow-network}

 \SetKwData{From}{from} \SetKwData{To}{to} \SetKwData{Length}{arc length}
    % \SetKwData{Capacity}{capacity} \SetKwData{Cost}{cost}
    \SetKwFunction{Capacity}{capacity} \SetKwFunction{Cost}{cost}
    \SetKwFunction{ShortestPathDist}{ShortestPathDist}
    \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
    
    \Input{ 
            $\bar{\mc{K}}^{*} = (\mc{F}^{*} \cup \mc{V}^{*}, \vec{\mc{E}}^{*} = \vec{\mc{E}}^{*}_{+} \cup \vec{\mc{E}}^{*}_{-} )$, 
            $\bm{z}^{*} \in \mc{Z}^{1}(\mc{K}^{*}; \integer) $,
            $\bm{c} \in \integer^{E}$, $\bm{a} \in \integer^{F}$, $\lambda \in \integerplus$ 
    }
    \Output{ 
            $\hat{\mc{K}}^{*}_{\vvec{\textsc{fn}}} 
                  = (\hat{\mc{F}}^{*}_{\vvec{\textsc{fn}}}, \hat{\mc{E}}^{*}_{\vvec{\textsc{fn}}})$ -- flow network for mSFN,
            % $\dist^{*}_{\bm{z}} \in \mc{C}^{0}(\mc{K}^{*}; \integer)$
    }
    \BlankLine
    
    % DIST LABELS
    \tcp*[h]{DIST LABELS of VOIDS $\equiv$ HOMOLOGY CLASS of $\bm{z}$}
    
    % $\dist(\bm{z}^{*}; \nu^{*}_{0}) \in \mc{C}^{0}(\mc{K}^{*}; \integer) \leftarrow$ 
    $\dist^{*}_{\bm{z}} \in \mc{C}^{0}(\mc{K}^{*}; \integer) \leftarrow$ 
    \ShortestPathDist {\From = $\nu^{*}_{0}$, \To = $\bar{\mc{F}}^{*}$, \Length = $\bm{z}^{*}$}\;
    \BlankLine
            % \To = $\mc{F}^{*}\setminus \{ \nu^{*}_{0} \}$, 

    % SOURCES - SINKS
    \tcp*[h]{VOIDS = SOURCES + TRANSITS + SINKS}
    
    $\mc{S} \leftarrow \big\{ \nu^{*}_{s} \in \mc{V}^{*} \mid \dist^{*}_{\bm{z}}(\nu^{*}_{s}) > 0   \big\}$,  
    $\mc{T} \leftarrow \big\{ \nu^{*}_{t} \in \mc{V}^{*} \mid \dist^{*}_{\bm{z}}(\nu^{*}_{t}) < 0   \big\}$,
    $\mc{Q} \leftarrow \emptyset$\;
    % $\mc{Q} \leftarrow \big\{ \nu^{*}_{k} \in \mc{V}^{*} \mid \dist^{*}_{\bm{z}}(\nu^{*}_{k}) = 0   \big\}$\; 
    \lIf { $\mc{S} \neq \emptyset$ and $\mc{T} = \emptyset$}{
            $\mc{T} \leftarrow \big\{ \nu^{*}_{t} \in \mc{V}^{*} \mid \dist^{*}_{\bm{z}}(\nu^{*}_{t}) = 0 \big\}$ 
    }
    \lElseIf{ $\mc{S} = \emptyset$ and $\mc{T} \neq \emptyset$}{
            $\mc{S} \leftarrow \big\{ \nu^{*}_{s} \in \mc{V}^{*} \mid \dist^{*}_{\bm{z}}(\nu^{*}_{s}) = 0 \big\}$ 
    }
    \lElse{
            $\mc{Q} \leftarrow \big\{ \nu^{*}_{k} \in \mc{V}^{*} \mid \dist^{*}_{\bm{z}}(\nu^{*}_{k}) = 0   \big\}$
    }
    \BlankLine


    % FLOW NETWORK
    \tcp*[h]{CONSTRUCT FLOW NETWORK}

    $\hat{\mc{F}}^{*}_{\vvec{\textsc{fn}}} \leftarrow \mc{F}^{*} \cup \mc{V}^{*} \cup \{ S^{*}, T^{*}, U^{*}, D^{*} \}$  
    \tcp*[f]{{\small facets*, voids*, \{source, sink, up, down\}}}
    
    $\vec{\mc{E}}^{*}_{\textsc{st}} \leftarrow 
%             \vec{\mc{E}}^{*}_{+} \cup \vec{\mc{E}}^{*}_{-}
            \vec{\mc{E}}^{*}
            \cup \{ (S^{*} \to \nu^{*}_k) \}_{\mc{S} \cup \mc{Q}}
            \cup \{ ( \nu^{*}_k \to T^{*}) \}_{\mc{T} \cup \mc{Q}}
            \cup \{ ( T^{*} \to S^{*}) \}
    $
    \tcp*[f]{OHCP network $\vec{\mc{K}}^{*}_{\textsc{st}}$}
    
   

    % $\tilde{\mc{E}}^{*} \leftarrow 
    %         \tilde{\mc{E}}^{*}
    %         \cup \{ (S^{*} \to U^{*}) \}
    %         \cup \{ (U^{*} \to \tau^{*}_j) \}_{\mc{F}^{*}}
    % $
    % \tcp*[f]{connect UP}

    % $\tilde{\mc{E}}^{*} \leftarrow 
    %         \tilde{\mc{E}}^{*}
    %         \cup \{ (D^{*} \to T^{*}) \}
    %         \cup \{ (\tau^{*}_j \to D^{*}) \}_{\mc{F}^{*}}
    % $
    % \tcp*[f]{connect DOWN}

    $\vec{\mc{E}}^{*}_{\textsc{u}} \leftarrow 
%            \{ (S^{*} \to U^{*}) \} \cup \{ (U^{*} \to \tau^{*}_j) \}_{\mc{F}^{*}}
            \{ (S^{*} \to U^{*}) \} \cup \{ (U^{*} \to \tau^{*}_j) \}_{j = 1}^{F}
    $
    % \tcp*[f]{$\cobd^{*}_{1}$UP}
    \tcp*[f]{up coboundary}

    $\vec{\mc{E}}^{*}_{\textsc{d}} \leftarrow 
            \{ (D^{*} \to T^{*}) \} \cup \{ (\tau^{*}_j \to D^{*}) \}_{\mc{F}^{*}}
    $
    % \tcp*[f]{$\cobd^{*}_{1}$DOWN}
    \tcp*[f]{down coboundary}

    $\hat{\mc{E}}^{*}_{\vvec{\textsc{fn}}} \leftarrow 
            % \vec{\mc{E}}^{*}_{+} \cup \vec{\mc{E}}^{*}_{-}
            \vec{\mc{E}}^{*}_{\textsc{st}} \cup \vec{\mc{E}}^{*}_{\textsc{u}} \cup \vec{\mc{E}}^{*}_{\textsc{d}}
            % \cup \{ (S^{*} \to \nu^{*}_k) \}_{\mc{S} \cup \mc{Q}}
            % \cup \{ ( \nu^{*}_k \to T^{*}) \}_{\mc{T} \cup \mc{Q}}
            % \cup \{ ( T^{*} \to S^{*}) \}
    $
    \tcp*[f]{FLAT-NORM network}



    % CAPACITIES AND COSTS
    \lForEach{$\vec{e}^{*}_{+i} \in \vec{\mc{E}}^{*}_{+}$}{
            \Cost {$\vec{e}^{*}_{+i}$} $\leftarrow  \bm{z}^{*}(\vec{e}^{*}_{+i}) \equiv \phantom{-} \bm{z}({e}_{i})$,
            \Capacity {$\vec{e}^{*}_{+i}$} $\leftarrow  c_i$,  
    }
    
    \lForEach{$\vec{e}^{*}_{-i} \in \vec{\mc{E}}^{*}_{-}$}{
            \Cost {$\vec{e}^{*}_{-i}$} $\leftarrow  \bm{z}^{*}(\vec{e}^{*}_{-i}) \equiv -\bm{z}({e}_{i})$,
            \Capacity {$\vec{e}^{*}_{-i}$} $\leftarrow  c_i$,  
    }

    
    \lForEach{$\vec{e}^{*} \in \{ \cobd^{*}_{1} S^{*} \} \cup \{ \cobd^{*}_{1} T^{*} \} $}{
            \Cost {$\vec{e}^{*}$} $\leftarrow  0$,
            \Capacity {$\vec{e}^{*}$} $\leftarrow  \infty$,  
    }

    \lForEach{$\vec{u}^{*}_j \in \tilde{\mc{E}}^{*}_{\textsc{u}} \setminus \{ (S^{*} \to U^{*}) \} $}{
            % \Capacity {$\vec{u}_j$} $\leftarrow  a^{\lambda}(\tau_{j}) = a^{\lambda}_j$,  
            \Cost {$\vec{u}^{*}_{j}$} $\leftarrow  0$,
            \Capacity {$\vec{u}^{*}_j$} $\leftarrow \lambda a_j$,  
    }

    \lForEach{$\vec{l}^{*}_j \in \tilde{\mc{E}}^{*}_{\textsc{d}} \setminus \{ (D^{*} \to T^{*}) \} $}{
            % \Capacity {$\vec{l}_j$} $\leftarrow  a^{\lambda}(\tau_{j}) = a^{\lambda}_j$,  
            \Cost {$\vec{l}^{*}_{j}$} $\leftarrow  0$,
            \Capacity {$\vec{l}^{*}_j$} $\leftarrow \lambda a_j$,  
    }


\end{algorithm}
%\DecMargin{1em}

